Search for lepton-flavour-violating decays of the Higgs and $Z$ bosons with the ATLAS detector

Direct searches for lepton flavour violation in decays of the Higgs and $Z$ bosons with the ATLAS detector at the LHC are presented. The following three decays are considered: $H\to e\tau$, $H\to\mu\tau$, and $Z\to\mu\tau$. The searches are based on the data sample of proton--proton collisions collected by the ATLAS detector corresponding to an integrated luminosity of 20.3 fb$^{-1}$ at a centre-of-mass energy of $\sqrt{s} = 8$ TeV. No significant excess is observed, and upper limits on the lepton-flavour-violating branching ratios are set at the 95% confidence level: Br$(H\to e\tau) <$ 1.04%, Br$(H\to\mu\tau) <$ 1.43%, and Br$(Z\to\mu\tau) <$ 1.69 $\times$ 10$^{-5}$.

==> Z_intro.tex <==
Additionally, the ATLAS data offer an interesting possibility to search for LFV in decays of Z boson \cite{DavidsonZ}. So far, such searches were performed at LEP \cite{PDG} for all channels and in ATLAS for $Z\to e\mu$ \cite{ATLASZemu}.  The Z boson decays are sensitive to a different LFV mechanism than decays of Higgs boson. If $H\to \ell_1 \ell_2$ is the only source of LFV one does not expect a signal in Z decays at measurable level \cite{HiggsLFVInZ} while other mechanism, e.g. heavy right handed neutrinos, could cause LFV in Z decays but not in Higgs decays \cite{NoHiggsInSeesaw}. The current upper limit on $Br(Z\to\tau\mu)$ is $1.2 \times 10^{-5}$ at 95\% CL.

%%% Local Variables:
%%% ispell-local-dictionary: ``british''
%%% End:

